Extrinsically-Focused Evaluation of Omissions in Medical Summarization

Large language models (LLMs) have shown promise in safety-critical applications such as healthcare, yet the ability to quantify performance has lagged. An example of this challenge is in evaluating a summary of the patient's medical record. A resulting summary can enable the provider to get a high-level overview of the patient's health status quickly. Yet, a summary that omits important facts about the patient's record can produce a misleading picture. This can lead to negative consequences on medical decision-making. We propose MED-OMIT as a metric to explore this challenge. We focus on using provider-patient history conversations to generate a subjective (a summary of the patient's history) as a case study. We begin by discretizing facts from the dialogue and identifying which are omitted from the subjective. To determine which facts are clinically relevant, we measure the importance of each fact to a simulated differential diagnosis. We compare MED-OMIT's performance to that of clinical experts and find broad agreement We use MED-OMIT to evaluate LLM performance on subjective generation and find some LLMs (gpt-4 and llama-3.1-405b) work well with little effort, while others (e.g. Llama 2) perform worse.

==> sections/limitations_ethics.tex <==
\section{Limitations}

We focus solely on omissions in this work but hope that future work can extend it to other potential summarization errors.  While using an extrinsic metric is less critical in detecting hallucinations given the presence of ground truth, summaries adding unneeded information could be detected using a similar approach.  Additionally, we detect an omission on a binary scale - either some part of the fact is omitted or none of it is.  An extension could include attempting to capture what percentage of the fact is omitted and the importance of the omitted aspect.  

Our metric pipeline performs best with a large LLM, such as gpt-4.  This adds increased cost when evaluating summaries.  While we feel this is warranted in safety-critical domains such as medicine, we also look towards exploring fine-tuned models to accomplish the same goals with reduced cost.  This is further an important goal as gpt-4 is a closed LLM, and having a high-performance open-source alternative is useful.

In addition, as a community, we need to invest in building more publicly available datasets. We were able to do this study only because of access to the openly available medical dialogue dataset. 

We use a publicly de-identified dataset for evaluating our approach.  However, given that this method can be applied to publicly available data, we caution that care should be taken when using non-hosted LLMs with sensitive data.  Additionally, while our approach is designed to aid a medical practitioner in making medical diagnoses, this is not designed to replace a medical practitioner overall.  
